Synthetic Examples Improve Generalization for Rare Classes

The ability to detect and classify rare occurrences in images has important applications - for example, counting rare and endangered species when studying biodiversity, or detecting infrequent traffic scenarios that pose a danger to self-driving cars. Few-shot learning is an open problem: current computer vision systems struggle to categorize objects they have seen only rarely during training, and collecting a sufficient number of training examples of rare events is often challenging and expensive, and sometimes outright impossible. We explore in depth an approach to this problem: complementing the few available training images with ad-hoc simulated data. Our testbed is animal species classification, which has a real-world long-tailed distribution. We analyze the effect of different axes of variation in simulation, such as pose, lighting, model, and simulation method, and we prescribe best practices for efficiently incorporating simulated data for real-world performance gain. Our experiments reveal that synthetic data can considerably reduce error rates for classes that are rare, that as the amount of simulated data is increased, accuracy on the target class improves, and that high variation of simulated data provides maximum performance gain.

==> authors.tex <==
Sara Beery*, Yang Liu*, Dan Morris$\circ$, Jim Piavis$\dagger$,\\ Ashish Kapoor$\dagger$, Markus Meister*, Neel Joshi$\dagger$, Pietro Perona*\\
\\
\begin{tabular}{cc}
California Institite of Technology* & Microsoft AI for Earth$\circ$, Microsoft Research$\dagger$\\
1200 E California Blvd, Pasadena, CA 91125 &
14820 NE 36th Street, Redmond, WA, 98052\\
\end{tabular}
